Comprehensive Privacy Analysis of Deep Learning: Passive and Active White-box Inference Attacks against Centralized and Federated Learning

Deep neural networks are susceptible to various inference attacks as they remember information about their training data. We design white-box inference attacks to perform a comprehensive privacy analysis of deep learning models. We measure the privacy leakage through parameters of fully trained models as well as the parameter updates of models during training. We design inference algorithms for both centralized and federated learning, with respect to passive and active inference attackers, and assuming different adversary prior knowledge. We evaluate our novel white-box membership inference attacks against deep learning algorithms to trace their training data records. We show that a straightforward extension of the known black-box attacks to the white-box setting (through analyzing the outputs of activation functions) is ineffective. We therefore design new algorithms tailored to the white-box setting by exploiting the privacy vulnerabilities of the stochastic gradient descent algorithm, which is the algorithm used to train deep neural networks. We investigate the reasons why deep learning models may leak information about their training data. We then show that even well-generalized models are significantly susceptible to white-box membership inference attacks, by analyzing state-of-the-art pre-trained and publicly available models for the CIFAR dataset. We also show how adversarial participants, in the federated learning setting, can successfully run active membership inference attacks against other participants, even when the global model achieves high prediction accuracies.

==> tab_active_all.tex <==
\begin{table}
\centering
 \caption{Accuracy of the active global attacker in the federated learning model.}
    \label{tab:active_all}
    
 \begin{tabular}{|c|c|c|}
    \hline
        \textbf{Dataset} & \textbf{Architecture} & \textbf{Attack Accuracy} \\
              \hline
        CIFAR100 & Alexnet & $93.1\%$\\
        CIFAR100 & DenseNet & $89.3\%$ \\
        Texas100 & Fully Connected & $71.7\%$ \\
        Purchase100 & Fully Connected & $82.5\%$ \\
        \hline
        \end{tabular}
   
\end{table}

==> tab_active_all_two_other.tex <==
\begin{table}
    \centering
     \caption{Accuracy of the active local attacker in the federated learning model.}
        \label{tab:active_all_two_other}
     \begin{tabular}{|c|c|c|}
        \hline
            \textbf{Dataset} & \textbf{Architecture} & \textbf{Attack Accuracy} \\
                  \hline
            CIFAR100 & Alexnet & $82.1\%$\\
            CIFAR100 & DenseNet & $79.3\%$ \\
            Texas100 & Fully Connected & $73.1\%$ \\
            Purchase100 & Fully Connected & $78.2\%$ \\
            \hline
            \end{tabular}
       
    \end{table}

==> tab_global_passive.tex <==



 

\begin{table}
\centering
\caption{The accuracy of the passive global attacker in the federated setting for various datasets and architectures. }
    \label{tab:global_passive}
 \begin{tabular}{|c|c|c|}
    \hline
        \textbf{Dataset} & \textbf{Architecture} & \textbf{Attack Accuracy} \\
    \hline
CIFAR100 & Alexnet & $89.0\%$ \\
        CIFAR100 & DenseNet & $84.3\%$ \\
        Texas100 & Fully Connected & $69.3\%$ \\
        Purchase100 & Fully Connected & $75.3\%$  \\
    \hline
        \end{tabular}
    
\end{table}

==> tab_local_passive.tex <==

\begin{table}
\centering
\caption{The accuracy of the passive local attacker in the federated learning model on different datasets and architectures.}
    \label{tab:local_passive}
 \begin{tabular}{|c|c|c|}
    \hline
        \textbf{Dataset} & \textbf{Architecture} & \textbf{Attack Accuracy} \\
              \hline
CIFAR100 & Alexnet & $70.4\%$ \\
        CIFAR100 & DenseNet & $69.8\%$ \\
        Texas100 & Fully Connected & $62.4\%$ \\
        Purchase100 & Fully Connected & $65.8\%$ \\
        \hline
        \end{tabular}
    
    \end{table}
    
